Bribe & Fork: Cheap Bribing Attacks via Forking Threat

In this work, we reexamine the vulnerability of Payment Channel Networks (PCNs) to bribing attacks, where an adversary incentivizes blockchain miners to deliberately ignore a specific transaction to undermine the punishment mechanism of PCNs. While previous studies have posited a prohibitive cost for such attacks, we show that this cost may be dramatically reduced (to approximately \$125), thereby increasing the likelihood of these attacks. To this end, we introduce Bribe & Fork, a modified bribing attack that leverages the threat of a so-called feather fork which we analyze with a novel formal model for the mining game with forking. We empirically analyze historical data of some real-world blockchain implementations to evaluate the scale of this cost reduction. Our findings shed more light on the potential vulnerability of PCNs and highlight the need for robust solutions.

==> figure-average.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}
\centering
\begin{subfigure}[][80pt][t]{.48\textwidth}
  \centering
  \caption{}
  \includegraphics[width=\textwidth]
{Average Fee.png}
  \label{fig:avfee}
\end{subfigure}
\begin{subfigure}[][80pt][t]{.48\textwidth}
  \centering
  \caption{}
  \includegraphics[width=\textwidth]
{Average Transaction Fee.png}
  \label{fig:avtxfree}
\end{subfigure}
\caption{\textbf{(a)} Average amount of fees aggregated in a block for each week in 2022 (\cite{btcexplorer}). \textbf{(b)} Average transaction fee of a single transaction for each week in 2022 (\cite{btcexplorer}).}
\label{fig:average}
\end{figure}
